A Taxonomy of Error Sources in HPC I/O Machine Learning Models

I/O efficiency is crucial to productivity in scientific computing, but the increasing complexity of the system and the applications makes it difficult for practitioners to understand and optimize I/O behavior at scale. Data-driven machine learning-based I/O throughput models offer a solution: they can be used to identify bottlenecks, automate I/O tuning, or optimize job scheduling with minimal human intervention. Unfortunately, current state-of-the-art I/O models are not robust enough for production use and underperform after being deployed. We analyze multiple years of application, scheduler, and storage system logs on two leadership-class HPC platforms to understand why I/O models underperform in practice. We propose a taxonomy consisting of five categories of I/O modeling errors: poor application and system modeling, inadequate dataset coverage, I/O contention, and I/O noise. We develop litmus tests to quantify each category, allowing researchers to narrow down failure modes, enhance I/O throughput models, and improve future generations of HPC logging and analysis tools.

==> figures/feature_table.tex <==
\begin{table}[ht] 
    \centering
    \caption{Condensed feature set and feature count}
    \begin{tabular}[t]{p{7.5cm} | >{\centering\arraybackslash}p{0.6cm} }
        \midrule
        \centering{Darshan features} & Count\\
        \midrule                                                                                                                                        
        $log_{10}$ of the job I/O throughput                                                                                                   & 1 \\
        $log_{10}$ of the total number of \{processes, files, accesses, bytes\}                                                                & 4 \\
        $log_{10}$ of the number of POSIX \{\texttt{open}, \texttt{seek}, \texttt{stat}, \texttt{mmap},& 6 \\
        \;\;\;\; \texttt{fsync}, \texttt{mode}\} calls  &   \\
        $log_{10}$ of \{memory, file\} alignment in bytes                                                                                      & 2 \\
        \% of all accesses that are \{reads, writes\}                                                                                          & 2 \\
        \% of all \{reads, writes\} that are \{consecutive, sequential\}                                                                       & 4 \\
        \% of all accesses that switch between reading and writing                                                                             & 1 \\
        \% of \{read, write\} accesses of size in ranges                                                                                       & 20 \\
        \;\;\;\;(0B, 100B], (100B, 1KiB], ..., (100MiB, 1GiB], (1GiB+)                 &  \\
        %\% of accesses in the \{1, 2, 3, 4\}-th most common access size                                                                       & 4 \\
        \% of non-aligned \{file, memory\} accesses                                                                                            & 2 \\ 
        \% of all bytes that are \{read, written\}                                                                                             & 2 \\
        \% of \{shared, unique, read-only, read-write, write-only\} files                                                                      & 5 \\
        \% of bytes read/written from \{shared, unique, read-only, read-write, write-only\} files                                              & 5 \\

        \midrule
        \centering{Lustre features (Cori only)} & Count\\
        \midrule                                                                                                                                        
        $log_{10}$ of file system \{byte, inode\} fullness \{min, mean, max, std\}  & 8 \\
        $log_{10}$ of metadata target \{closes, getattrs, getxattrs, links, mkdirs, mknods, opens, renames, rmdirs, setattrs, statfss,
        unlinks\} operation mean & 12 \\
        \% of data server \{CPU, memory\} \{min, mean, max, std\}          & 8 \\
        \% of data target bytes \{read, written\} \{min, mean, max, std\}  & 8 \\
        \% of metadata server CPU usage \{min, mean, max, std\}            & 1 \\

        \midrule
        \centering{Cobalt features (Theta only)} & Count\\
        \midrule                                                                                                                                               
        $log_{10}$ of \{core, node\} count                                 & 2 \\
        $log_{10}$ of job runtime                                          & 1 \\
        \% of job \{start, end\} time relative to total system timerange   & 2\\ 
        \midrule

    \end{tabular}\label{table:features}
\end{table}%


